Multi-wavelength study of TeV blazar 1ES 1218+304 using gamma-ray, X-ray and optical observations

We report the multi-wavelength study for a high-synchrotron-peaked BL Lac 1ES 1218+304 using near-simultaneous data obtained during the period from January 1, 2018, to May 31, 2021 (MJD 58119-59365) from various instruments including Fermi-LAT, Swift-XRT, AstroSat, and optical from Swift-UVOT $\&$ TUBITAK observatory in Turkey. The source was reported to be flaring in TeV $\gamma$-ray band during 2019, but no significant variation is observed with Fermi-LAT. A sub-hour variability is seen in the SXT light curve, suggesting a compact emission region for their variability. However, hour scale variability is observed in the $\gamma$-ray light curve. A "softer-when-brighter" trend is observed in $\gamma$-rays, and an opposite trend is seen in X-rays suggesting both emissions are produced via two different processes as expected from an HBL source. We have chosen the two epochs in January 2019 to study and compare their physical parameters. A joint fit of SXT and LAXPC provides a constraint on the synchrotron peak, roughly estimated to be $\sim$1.6 keV. A clear shift in the synchrotron peak is observed from $\sim$1 keV to above 10 keV revealing its extreme nature or behaving like an EHBL-type source. The optical observation provides color-index variation as "blue-when-brighter". The broadband SED is fitted with a single-zone SSC model, and their parameters are discussed in the context of a TeV blazar and the possible mechanism behind the broadband emission.

==> Figures/Extra_plots.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{Figures/index_3.pdf}
\caption{\textcolor{blue}{Scatter plot for the correlation between Flux and Index of the blazar 1ES 1218+304. Top plot represents the 7-day binned Fermi-Lat data. The slope is positive and Person correlation coefficient is 0.595. Bottom plot represents Swift-XRT data for Flux (0.3-10 KeV) vs Photon Index. The slope is negative and Pearson correlation coefficient is -0.748, it follows an inverse trend as the $\gamma$-ray data. The orange line is a linear fit for reference.}}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[height=\linewidth, angle=270,trim={2cm 1cm 2cm 5cm},clip]{Figures/lc_100.pdf}
\caption{100 Sec binned lightcurve from LAXPC instrument}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[height=\linewidth, angle=270,trim={2cm 1cm 2cm 5cm},clip]{Figures/lc_50.pdf}
\caption{50 Sec binned lightcurve from LAXPC instrument}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[height=\linewidth, angle=270,trim={2cm 1cm 2cm 5cm},clip]{Figures/lc_1.pdf}
\caption{1 Sec binned lightcurve from LAXPC instrument}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
\end{center}
\end{figure}


%\begin{figure*}
%\begin{center}
%\includegraphics[width=7in]{Figures/lc_7_2.pdf}
%\caption{\textcolor{blue}{Multi-wavelength light curve of 1ES 1218+304 from January 2018 to June 2021. The $\gamma$-ray flux are presented in units of 10$^{-8}$ ph cm$^{-2}$ s$^{-1}$, and X-ray fluxes are in units of 10$^{-10}$ erg cm$^{-2}$ s$^{-1}$. The vertical red line represents the Flare period from 5-7 January, 2019 and vertical green line represents the Flare period from 15-20 January, 2019. This period also includes the data from \texttt{AstroSat} Data from 17-20 January, 2019. }}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=7in]{Figures/lc_7_1.pdf}
%\caption{\textcolor{blue}{Multi-wavelength light curve of 1ES 1218+304 from January 2018 to June 2021. The $\gamma$-ray flux are presented in units of 10$^{-8}$ ph cm$^{-2}$ s$^{-1}$, and X-ray fluxes are in units of 10$^{-10}$ erg cm$^{-2}$ s$^{-1}$. The vertical red line represents the Flare period from 5-7 January, 2019 and vertical green line represents the Flare period from 15-20 January, 2019. This period also includes the data from \texttt{AstroSat} Data from 17-20 January, 2019. }}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure*}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=7in]{Figures/lc_15_2.pdf}
%\caption{\textcolor{blue}{Multi-wavelength light curve of 1ES 1218+304 from January 2018 to June 2021. The $\gamma$-ray flux are presented in units of 10$^{-8}$ ph cm$^{-2}$ s$^{-1}$, and X-ray fluxes are in units of 10$^{-10}$ erg cm$^{-2}$ s$^{-1}$. The vertical red line represents the Flare period from 5-7 January, 2019 and vertical green line represents the Flare period from 15-20 January, 2019. This period also includes the data from \texttt{AstroSat} Data from 17-20 January, 2019. }}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure*}


%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{index.pdf}
%\caption{Shadow of a Schwarzschild BH and a Kerr BH}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[width=\linewidth]{index_1.pdf}
%\caption{Shadow of a Schwarzschild BH and a Kerr BH}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure}

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.73\linewidth, height=0.73\linewidth]{Screenshot from 2021-10-22 16-50-27.png}
%\caption{Shadow of a Schwarzschild BH and a Kerr BH}
%\label{fig:kerr}
%The observer is a at infinity in the equatorial plane.
%\end{center}
%\end{figure}

